Projected Off-Policy Q-Learning (POP-QL) for Stabilizing Offline Reinforcement Learning

A key problem in off-policy Reinforcement Learning (RL) is the mismatch, or distribution shift, between the dataset and the distribution over states and actions visited by the learned policy. This problem is exacerbated in the fully offline setting. The main approach to correct this shift has been through importance sampling, which leads to high-variance gradients. Other approaches, such as conservatism or behavior-regularization, regularize the policy at the cost of performance. In this paper, we propose a new approach for stable off-policy Q-Learning. Our method, Projected Off-Policy Q-Learning (POP-QL), is a novel actor-critic algorithm that simultaneously reweights off-policy samples and constrains the policy to prevent divergence and reduce value-approximation error. In our experiments, POP-QL not only shows competitive performance on standard benchmarks, but also out-performs competing methods in tasks where the data-collection policy is significantly sub-optimal.

==> tables/d4rl_adv_results.tex <==
\begin{tabular}{l||rrrr}
 & SAC-off & BC & CQL & POP-QL \\
\hline
halfcheetah-adv-random & \bfseries 18.46 & -83.85 & 2.68 & 3.60 \\
halfcheetah-adv-medium & \bfseries 51.30 & -97.09 & 43.23 & nan \\
halfcheetah-adv-expert & 1.60 & -101.03 & \bfseries 26.78 & 2.95 \\
hopper-adv-random & \bfseries 8.13 & 0.54 & 0.53 & 6.25 \\
hopper-adv-medium & \bfseries 1.79 & 0.53 & 0.53 & nan \\
hopper-adv-expert & 3.37 & 0.54 & 0.53 & \bfseries 8.28 \\
walker2d-adv-random & 5.62 & -0.72 & \bfseries 7.77 & 0.07 \\
walker2d-adv-medium & 0.04 & -0.72 & \bfseries 82.11 & nan \\
walker2d-adv-expert & 0.35 & -0.72 & \bfseries 115.75 & 0.33 \\
\end{tabular}


==> tables/d4rl_max.tex <==
\begin{tabular}{l||rrrrrr}
& SAC-off & BEAR* & BCQ* & aDICE* & CQL & POP-QL \\
\hline
maze2d-umaze & 548.93 & 3.40 & 12.80 & -15.70 & 321.30 & \bfseries 595.60 \\
maze2d-medium & 242.95 & 29.00 & 8.30 & 10.00 & 82.77 & \bfseries 243.28 \\
maze2d-large & 240.21 & 4.60 & 6.20 & -0.10 & 171.71 & \bfseries 249.34 \\
\hline
hopper-random & 33.09 & 9.50 & 10.60 & 0.90 & 5.56 & \bfseries 34.19 \\
halfcheetah-random & 29.33 & 25.50 & 2.20 & -0.30 & 2.28 & \bfseries 31.06 \\
walker2d-random & \bfseries 17.34 & 6.70 & 4.90 & 0.50 & 5.25 & 12.61 \\
\hline
hopper-medium & 9.24 & 47.60 & 54.50 & 1.20 & 53.56 & \bfseries 85.12 \\
halfcheetah-medium & 59.00 & 38.60 & 40.70 & -2.20 & \bfseries 63.64 & 45.15 \\
walker2d-medium & 6.65 & 33.20 & 53.10 & 0.30 & 21.45 & \bfseries 62.79 \\
\hline
hopper-medium-replay & 90.04 & \bfseries 96.30 & 33.10 & 1.10 & 17.84 & 68.68 \\
halfcheetah-medium-replay & \bfseries 53.91 & 38.60 & 38.20 & -0.80 & 52.10 & 39.04 \\
walker2d-medium-replay & 53.61 & 19.20 & 15.00 & 0.60 & \bfseries 78.61 & 35.17 \\
\hline
hopper-medium-expert & 13.20 & 4.00 & \bfseries 110.90 & 1.10 & 56.11 & 57.16 \\
halfcheetah-medium-expert & 12.33 & 51.70 & 64.70 & -0.80 & \bfseries 89.70 & 54.51 \\
walker2d-medium-expert & 8.44 & 10.80 & 57.50 & 0.40 & \bfseries 93.66 & 75.46 \\
\hline
antmaze-umaze & 13.00 & 73.00 & \bfseries 78.90 & 0.00 & 16.82 & 58.50 \\
antmaze-medium-play & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & \bfseries 29.50 \\
antmaze-large-play & 0.00 & 0.00 & \bfseries 6.70 & 0.00 & 0.00 & 0.00 \\
antmaze-umaze-diverse & 0.00 & \bfseries 61.00 & 55.00 & 0.00 & 8.33 & 0.00 \\
antmaze-medium-diverse & 2.50 & 8.00 & 0.00 & 0.00 & 7.92 & \bfseries 19.00 \\
antmaze-large-diverse & \color{red}{nan} & 0.00 & \bfseries 2.20 & 0.00 & 0.00 & 0.00 \\
\hline
kitchen-complete & 28.25 & 0.00 & 8.10 & 0.00 & 26.62 & \bfseries 31.62 \\
kitchen-partial & 24.12 & 13.10 & 18.90 & 0.00 & \bfseries 29.62 & 27.25 \\
kitchen-mixed & 23.88 & \bfseries 47.20 & 8.10 & 0.00 & 24.75 & 32.38 \\
\end{tabular}


==> tables/d4rl_results.tex <==
\begin{tabular}{l||rrrrrr}
& SAC-off & BEAR* & BCQ* & aDICE* & CQL & POP-QL (ours) \\
\hline
maze2d-umaze & \bfseries 446.87 & 3.40 & 12.80 & -15.70 & 278.85 & 89.09 \\
maze2d-medium & \bfseries 150.68 & 29.00 & 8.30 & 10.00 & 54.95 & 96.44 \\
maze2d-large & 122.26 & 4.60 & 6.20 & -0.10 & 17.73 & \bfseries 147.76 \\
\hline
hopper-random & 11.88 & 9.50 & 10.60 & 0.90 & 0.92 & \bfseries 12.68 \\
hopper-medium & 2.32 & 47.60 & \bfseries 54.50 & 1.20 & 44.71 & 33.30 \\
hopper-medium-replay & 18.54 & \bfseries 96.30 & 33.10 & 1.10 & 2.05 & 32.07 \\
hopper-medium-expert & 2.31 & 4.00 & \bfseries 110.90 & 1.10 & 45.72 & 8.76 \\
halfcheetah-random & 27.97 & 25.50 & 2.20 & -0.30 & -1.12 & \bfseries 31.01 \\
halfcheetah-medium & 57.28 & 38.60 & 40.70 & -2.20 & \bfseries 62.37 & 43.54 \\
halfcheetah-medium-replay & 43.34 & 38.60 & 38.20 & -0.80 & \bfseries 50.03 & 35.06 \\
halfcheetah-medium-expert & 6.41 & 51.70 & 64.70 & -0.80 & \bfseries 82.76 & 58.93 \\
walker2d-random & 4.55 & \bfseries 6.70 & 4.90 & 0.50 & -0.02 & 0.73 \\
walker2d-medium & 0.94 & 33.20 & \bfseries 53.10 & 0.30 & 7.36 & 8.41 \\
walker2d-medium-replay & 5.05 & 19.20 & 15.00 & 0.60 & \bfseries 63.97 & 23.01 \\
walker2d-medium-expert & 0.08 & 10.80 & \bfseries 57.50 & 0.40 & 10.12 & 1.60 \\
\hline
antmaze-umaze & 3.50 & 73.00 & \bfseries 78.90 & 0.00 & 8.50 & 32.00 \\
antmaze-umaze-diverse & 0.00 & \bfseries 61.00 & 55.00 & 0.00 & 0.00 & 0.00 \\
antmaze-medium-play & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & \bfseries 0.50 \\
antmaze-medium-diverse & 0.00 & \bfseries 8.00 & 0.00 & 0.00 & 0.00 & 2.50 \\
antmaze-large-play & 0.00 & 0.00 & \bfseries 6.70 & 0.00 & 0.00 & 0.00 \\
antmaze-large-diverse & nan & 0.00 & \bfseries 2.20 & 0.00 & 0.00 & 0.00 \\
\hline
kitchen-complete & 0.12 & 0.00 & \bfseries 8.10 & 0.00 & 0.00 & nan \\
kitchen-partial & 0.00 & 13.10 & \bfseries 18.90 & 0.00 & 6.12 & nan \\
kitchen-mixed & 0.00 & \bfseries 47.20 & 8.10 & 0.00 & 0.62 & nan \\
\end{tabular}


==> tikz_settings.tex <==
\definecolor{viridis00}{RGB}{253, 231, 37}
\definecolor{viridis01}{RGB}{181, 222, 43}
\definecolor{viridis02}{RGB}{110, 206, 88}
\definecolor{viridis03}{RGB}{53, 183, 121}
\definecolor{viridis04}{RGB}{31, 158, 137}
\definecolor{viridis05}{RGB}{38, 130, 142}
\definecolor{viridis06}{RGB}{49, 104, 142}
\definecolor{viridis07}{RGB}{62, 73, 137}
\definecolor{viridis08}{RGB}{72, 40, 120}
\definecolor{viridis09}{RGB}{68, 1, 84}

\definecolor{datapolicy}{RGB}{135, 93, 145}
\definecolor{optimpolicy}{RGB}{80, 135, 173}

\definecolor{poptdraw}{RGB}{38, 130, 142}
\colorlet{poptd}{black!30!poptdraw}
\colorlet{poptds}{white!70!poptdraw}

\definecolor{naivetdraw}{RGB}{72, 40, 120}
\colorlet{naivetd}{black!30!naivetdraw}
\colorlet{naivetds}{white!70!naivetdraw}

\definecolor{dualdiceraw}{RGB}{110, 206, 88}
\colorlet{dualdice}{black!30!dualdiceraw}
